Large-scale empirical study on the momentum equation's inertia term

A common approach to reduce the Euler equations' complexity for the simulation and optimization of gas networks is to neglect small terms that contribute little to the overall equations. An example is the inertia term of the momentum equation since it is said to be of negligible size under real-world operating conditions. However, this justification has always only been based on experience or single sets of artificial data points. This study closes this gap by presenting a large-scale empirical evaluation of the absolute and relative size of the inertia term when operating a real-world gas network. Our data consists of three years of fine-granular state data of one of the largest gas networks in Europe, featuring over 6,000 pipes with a total length of over 10,000 km. We found that there are only 120 events in which a subnetwork consisting of multiple pipes has an inertia term of high significance for more than three minutes. On average, such an event occurs less often than once every ten days. Therefore, we conclude that the inertia term is indeed negligible for real-world transient gas network control problems.

==> commands.tex <==
\RequirePackage{xspace}
\RequirePackage{accents}

%%-------------------------------------------------------------
%% Abbreviations
%%-------------------------------------------------------------
\newcommand{\myie}{i.e.}
\newcommand{\myIe}{I.e.}
\newcommand{\myeg}{e.g.}
\newcommand{\myst}{s.t.\ }
\newcommand{\myWlog}{W.l.o.g.\ }
\newcommand{\mywlog}{w.l.o.g.\ }
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% nice underbar, needs 'accents' package
%\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}
\newcommand{\ubar}[1]{\underaccent{\bar}{{#1}}}

\newcommand{\ub}[1]{\ensuremath{\bar{#1}}\xspace}
\newcommand{\lb}[1]{\ensuremath{\ubar{#1}}\xspace}

\newcommand{\powerset}{\ensuremath{\mathcal{P}}\xspace}
% set of halfspaces representing the faces of some polytope (compressor config polytope, tv bound polytope, etc.)
\newcommand{\setFacets}[1]{\ensuremath{\mathcal{H}_{#1}}\xspace}

%%----------------------------------------------------------
%% all used mathcal letters
%%----------------------------------------------------------
% A - arcs
% C - compressor configurations
% F - flow directions
% G - fence groups
% H - configuration facets(hyperplanes)
% M - machines (maybe unify with U?)
% O - operation modes
% P - power set
% Q - valid operation mode/flowdirection combinations
% S - Simple states
% T - time steps
% U - units (maybe unify with M?)
% V - vertices
% W - flow direction conditions

%%-----------------------------------------------------------
%% Graph
%%----------------------------------------------------------
\newcommand{\graph}{\ensuremath{G}\xspace}
\newcommand{\generalGraph}{\ensuremath{\graph=(\setVertices,\setArcs)}\xspace}
\newcommand{\netmodelGraph}{\ensuremath{\graph=(\setVertices,\setPipes \cup \setRegulators \cup \setValves \cup \setArtificialLinks)}\xspace}

% nodes
\newcommand{\setVertices}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\setVerticesAll}{\ensuremath{\setVertices = \setBoundaryNodes \cup \setInnerNodes}\xspace}
\newcommand{\setEntries}{\ensuremath{\setVertices^{+}}\xspace}
\newcommand{\setExits}{\ensuremath{\setVertices^{-}}\xspace}
\newcommand{\setBoundaryNodes}{\ensuremath{\setVertices^\mathrm{b}}\xspace}
\newcommand{\setBoundaryNodesAll}{\ensuremath{\setEntries \cup \setExits}\xspace}
\newcommand{\setInnerNodes}{\ensuremath{\setVertices^{0}}\xspace}
\newcommand{\setFenceNodes}{\ensuremath{\setVertices^{\mathrm{fn}}}\xspace}
\newcommand{\setFenceNodesNaviStation}[1]{\ensuremath{\setFenceNodes_{i}}\xspace}
\newcommand{\setArtificialNodes}{\ensuremath{\setVertices^{\mathrm{ar}}}\xspace}
\newcommand{\setArtificialNodesNaviStation}[1]{\ensuremath{\setArtificialNodes_{#1}}\xspace}

% arcs
\newcommand{\setArcs}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\setArcsAllStationModel}{\ensuremath{\setArcs = \setPipes \cup \setValves \cup \setResistors \cup \setRegulators \cup \setCompressorStations}\xspace}
\newcommand{\setPipes}{\ensuremath{\setArcs^{\mathrm{pi}}}\xspace}
\newcommand{\setRegulators}{\ensuremath{\setArcs^{\mathrm{rg}}}\xspace}
\newcommand{\setValves}{\ensuremath{\setArcs^{\mathrm{va}}}\xspace}
\newcommand{\setValvesNS}{\ensuremath{\setArcs^{\mathrm{va-s}}}\xspace}
\newcommand{\setResistors}{\ensuremath{\setArcs^{\mathrm{rs}}}\xspace}
\newcommand{\setCompressorStations}{\ensuremath{\setArcs^{\mathrm{cs}}}\xspace}

% station model specific arcs
\newcommand{\setRegulatorsControllable}{\ensuremath{\setArcs^{\mathrm{rg-c}}}\xspace}
\newcommand{\setRegulatorsNonControllable}{\ensuremath{\setArcs^{\mathrm{rg-nc}}}\xspace}
\newcommand{\setRegulatorsNonControllableActive}{\ensuremath{\setArcs^{\mathrm{rg-nca}}}\xspace}
\newcommand{\setRegulatorsNonControllableFixed}{\ensuremath{\setArcs^{\mathrm{rg-ncf}}}\xspace}
\newcommand{\setRegulatorsNonControllableAll}{\ensuremath{\setRegulatorsNonControllable := \setRegulatorsNonControllableActive\cup\setRegulatorsNonControllableFixed}\xspace}

% special compressor station sets
\newcommand{\setCompressorUnits}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\setCompressorUnitsI}[1]{\ensuremath{\setCompressorUnits_{#1}}\xspace}
\newcommand{\setCompressorConfigurations}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setCompressorConfigurationsUsingUnit}[1]{\ensuremath{\mathcal{C}_{#1}}\xspace}
\newcommand{\setConfigurationFacets}[1]{\ensuremath{\setFacets{#1}}\xspace}

% navi station specific (net model)
\newcommand{\naviStationGraph}[1]{\ensuremath{G}_{#1}\xspace}
\newcommand{\naviStationGraphAll}[1]{\ensuremath{\naviStationGraph{#1}=(\setVerticesNaviStation{#1},\setArtificialLinksNaviStation{#1})\xspace}}
\newcommand{\setVerticesNaviStation}[1]{\ensuremath{\setVertices}_{#1}\xspace}
\newcommand{\setArtificialLinksNaviStation}[1]{\ensuremath{\setArcs^{\mathrm{ar}}}_{#1}\xspace}
\newcommand{\nNaviStations}{\ensuremath{m}\xspace}

% navi station specific (station model)
\newcommand{\setNSModes}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\setNSValidPairs}{\ensuremath{\mathcal{Q}}\xspace} % valid pairs of operation modes and flow directions
\newcommand{\setNSFenceGroups}{\ensuremath{\mathcal{G}}\xspace}
% old commands, deprecated, just used to create the latexdiff for the stationModelPaper
\newcommand{\setOldNSValidPairs}{\ensuremath{\mathcal{OF}}\xspace}
\newcommand{\setOldNSFenceGroups}{\ensuremath{\mathcal{FG}}\xspace}
% end of old commands
\newcommand{\setBoundaryNodesExitP}{\ensuremath{\setVertices^\mathrm{b-ex}}\xspace}

%%-----------------------------------------------------------
%% Time
%%----------------------------------------------------------
\newcommand{\setTimesteps}{\ensuremath{\mathcal{T}_0}\xspace}
\newcommand{\setTimestepsNoZero}{\ensuremath{\mathcal{T}}\xspace}
\newcommand{\nTimesteps}{\ensuremath{k}\xspace}
\newcommand{\setTimestepsAll}{\ensuremath{\setTimesteps := \{0, \dots, \nTimesteps\}}\xspace}
\newcommand{\setTimestepsNoZeroAll}{\ensuremath{\setTimestepsNoZero := \setTimesteps\setminus\{0\}}\xspace}
\newcommand{\granularity}{\ensuremath{\tau}\xspace}
\newcommand{\granularityI}[1]{\ensuremath{\granularity(#1)}\xspace}

%%-----------------------------------------------------------
%% Supplies and demands
%%----------------------------------------------------------
\newcommand{\inflow}{\ensuremath{d}}
\newcommand{\paramInflowValue}[2]{\ensuremath{D_{#1,#2}}\xspace}
\newcommand{\paramSupplyValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramDemandValue}[2]{\ensuremath{\paramInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \paramInflowValue
\newcommand{\paramSupplyUB}[2]{\ensuremath{\ub{D}_{#1,#2}}\xspace}
\newcommand{\paramDemandUB}[2]{\ensuremath{\lb{D}_{#1,#2}}\xspace}
\newcommand{\inflowI}[1]{\ensuremath{\inflow_{#1}}\xspace}
\newcommand{\paramInflowValueUB}[2]{\ensuremath{\ub{\inflow}_{#1,#2}}\xspace}
\newcommand{\paramInflowValueLB}[2]{\ensuremath{\lb{\inflow}_{#1,#2}}\xspace}
\newcommand{\varSupplyValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue
\newcommand{\varDemandValue}[2]{\ensuremath{\varInflowValue{#1}{#2}}\xspace} %TODO Kai: replace by \varInflowValue

% station model demands for inflow and pressure
\newcommand{\demandPressure}[1]{\ensuremath{\hat{\press}_{#1}}\xspace}
\newcommand{\demandInflow}[1]{\ensuremath{\hat{\inflow}_{#1}}\xspace}

%%-----------------------------------------------------------
%% Pressure
%%----------------------------------------------------------
\newcommand{\press}{\ensuremath{p}\xspace}
\newcommand{\pressI}[1]{\ensuremath{\press_{#1}}\xspace}
\newcommand{\pressUB}[1]{\ensuremath{\ub{\press}_{#1}}\xspace}
\newcommand{\pressLB}[1]{\ensuremath{\lb{\press}_{#1}}\xspace}
\newcommand{\inflowPressUB}[1]{\ensuremath{\paramPressUB{#1}^{\mathrm{act}}}\xspace} % act => active
\newcommand{\inflowPressLB}[1]{\ensuremath{\paramPressLB{#1}^{\mathrm{act}}}\xspace} % act => active

%%-----------------------------------------------------------
%% Flow
%%----------------------------------------------------------
\newcommand{\mFlow}{\ensuremath{q}\xspace}
\newcommand{\mFlowI}[1]{\ensuremath{\mFlow_{#1}}\xspace}
\newcommand{\mFlowFwd}[1]{\ensuremath{\mFlow{#1}^{\rightarrow}}\xspace}
\newcommand{\mFlowBwd}[1]{\ensuremath{\mFlow{#1}^{\leftarrow}}\xspace}
\newcommand{\mFlowUB}[1]{\ensuremath{\ub{\mFlow}_{#1}}\xspace}
\newcommand{\mFlowLB}[1]{\ensuremath{\lb{\mFlow}_{#1}}\xspace}
\newcommand{\fenceFlow}[1]{\ensuremath{\varArcFlow{#1}^\mathrm{fn}}\xspace}

%%-----------------------------------------------------------
%% Netmodel Navi Station
%%----------------------------------------------------------
\newcommand{\setArtificialLinks}{\ensuremath{\setArcs^{\mathrm{ar}}}\xspace}
\newcommand{\setShortcuts}{\ensuremath{\setArcs^{\mathrm{ar-sc-bi}}}\xspace}
\newcommand{\setShortcutsNaviStation}[1]{\ensuremath{\setShortcuts_{#1}}\xspace}
\newcommand{\setRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg}}}\xspace}
\newcommand{\setRegulatorArcsNaviStation}[1]{\ensuremath{\setRegulatorArcs_{#1}}\xspace}
\newcommand{\setCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp}}}\xspace}
\newcommand{\setCompressorArcsNaviStation}[1]{\ensuremath{\setCompressorArcs_{#1}}\xspace}
\newcommand{\setCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb}}}\xspace}
\newcommand{\setCombinedArcsNaviStation}[1]{\ensuremath{\setCombinedArcs_{#1}}\xspace}

\newcommand{\setBiRegulatorArcs}{\ensuremath{\setArcs^{\mathrm{ar-rg-bi}}}\xspace}
\newcommand{\setBiRegulatorArcsNaviStation}[1]{\ensuremath{\setBiRegulatorArcs_{#1}}\xspace}
\newcommand{\setBiCompressorArcs}{\ensuremath{\setArcs^{\mathrm{ar-cp-bi}}}\xspace}
\newcommand{\setBiCompressorArcsNaviStation}[1]{\ensuremath{\setBiCompressorArcs_{#1}}\xspace}
\newcommand{\setBiCombinedArcs}{\ensuremath{\setArcs^{\mathrm{ar-cb-bi}}}\xspace}
\newcommand{\setBiCombinedArcsNaviStation}[1]{\ensuremath{\setBiCombinedArcs_{#1}}\xspace}

\newcommand{\setDirectedArcs}{\ensuremath{\setArcs^{\mathrm{ar-di}}}\xspace}
\newcommand{\setDirectedArcsNaviStation}[1]{\ensuremath{\setDirectedArcs_{#1}}\xspace}
\newcommand{\setBiArcs}{\ensuremath{\setArcs^{\mathrm{ar-bi}}}\xspace}
\newcommand{\setBiArcsNaviStation}[1]{\ensuremath{\setBiArcs_{#1}}\xspace}
\newcommand{\setCompressingArcs}{\ensuremath{\setArcs^{\mathrm{ar-co}}}\xspace}
\newcommand{\setCompressingArcsNaviStation}[1]{\ensuremath{\setCompressingArcs_{#1}}\xspace}

\newcommand{\setSimpleStates}{\ensuremath{\mathcal{S}}\xspace}
\newcommand{\setSimpleStatesNaviStation}[1]{\ensuremath{\mathcal{S}_{#1}}\xspace}
\newcommand{\simpleState}{\ensuremath{s}\xspace}
\newcommand{\simpleStateFlowDirections}{\ensuremath{\simpleState^{\flowDirection}}\xspace}
\newcommand{\simpleStateLinksMandatoryActive}{\ensuremath{\simpleState^{on}}\xspace}
\newcommand{\simpleStateLinksMandatoryInactive}{\ensuremath{\simpleState^{off}}\xspace}

\newcommand{\varActivation}[2]{\ensuremath{x_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varSimpleStateActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivation}[2]{\ensuremath{\varActivation{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkActivationFwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\rightarrow}}\xspace}
\newcommand{\varArtificialLinkActivationBwd}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\leftarrow}}\xspace}
\newcommand{\varCombinedLinkRegulatingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{rg}}}\xspace}
\newcommand{\varCombinedLinkCompressingActivation}[2]{\ensuremath{\varArtificialLinkActivation{#1}{#2}^{\mathrm{cp}}}\xspace}

\newcommand{\varChange}[2]{\ensuremath{\delta_{#1,#2}}\xspace}
\newcommand{\varFlowDirectionChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varSimpleStateChange}[2]{\ensuremath{\varChange{#1}{#2}}\xspace}
\newcommand{\varArtificialLinkChangeOn}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{on}}}\xspace}
\newcommand{\varArtificialLinkChangeOff}[2]{\ensuremath{\varChange{#1}{#2}^{\mathrm{off}}}\xspace}

\newcommand{\setFlowDirectionConditions}{\ensuremath{\mathcal{W}}\xspace}
\newcommand{\setFlowDirectionConditionsNaviStation}[1]{\ensuremath{\setFlowDirectionConditions_{i}}\xspace}

%%-----------------------------------------------------------
%% Machines, Power, Compression Ratio, and Betriebsvolumenstrom
%%-----------------------------------------------------------
\newcommand{\setMachinesNaviStation}[1]{\ensuremath{\mathcal{M}}_{#1}\xspace}
\newcommand{\setMachinesNaviStationOnLink}[2]{\ensuremath{\setMachinesNaviStation{#1}^{#2}}\xspace}
\newcommand{\generalMachine}{\ensuremath{m}\xspace}
\newcommand{\machine}[1]{\ensuremath{\generalMachine_{#1}}\xspace}

\newcommand{\varAssignMachineToLink}[3]{\ensuremath{y_{#1,#2,#3}}\xspace}

\newcommand{\paramMaxNumberMachinesLink}{\ensuremath{M_a^{\mathrm{max}}}\xspace}
\newcommand{\paramMaxCompressionRatio}[2]{\ensuremath{R_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxPower}[2]{\ensuremath{\power_{\machine{#1},#2}}\xspace}
\newcommand{\paramMaxBetriebsVolumenstrom}[2]{\ensuremath{\volumetricFlow_{\machine{#1},#2}}\xspace}

\newcommand{\varCompressionRatio}[2]{\ensuremath{r_{#1,#2}}\xspace}
\newcommand{\varPower}[2]{\ensuremath{\pi_{#1,#2}}\xspace}
\newcommand{\varBetriebsVolumenstrom}[2]{\ensuremath{\omega_{#1,#2}}\xspace}
\newcommand{\varMaxPower}[2]{\ensuremath{\varPower{#1}{#2}^{max}}\xspace}
\newcommand{\varMaxBetriebsVolumenstrom}[2]{\ensuremath{\varBetriebsVolumenstrom{#1}{#2}^{max}}\xspace}

\newcommand{\paramMaxCompressionRatioLink}[2]{\ensuremath{\ub{R}_{#1,#2}}\xspace}
\newcommand{\paramPressureUBCompression}[2]{\ensuremath{\paramPressureUB{#1}{#2}^{\mathrm{out}}}\xspace}


%%-----------------------------------------------------------
%% Smoothing
%%-----------------------------------------------------------

\newcommand{\generalSmoothing}{\ensuremath{\delta}\xspace}
\newcommand{\varSmoothingPressurePos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press+}}\xspace}
\newcommand{\varSmoothingPressureNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\press-}}\xspace}
\newcommand{\varSmoothingInflowPos}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow+}}\xspace}
\newcommand{\varSmoothingInflowNeg}[2]{\ensuremath{\generalSmoothing_{#1,#2}^{\mFlow-}}\xspace}

%%-----------------------------------------------------------
%% Flow Direction (used in both models)
%%-----------------------------------------------------------
\newcommand{\setFlowDirectionsNavi}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\setFlowDirectionsNaviStation}[1]{\ensuremath{\setFlowDirectionsNavi_{#1}}\xspace}
\newcommand{\flowDirection}{\ensuremath{f}\xspace}
\newcommand{\flowDirectionEntries}{\ensuremath{\flowDirection^{+}}\xspace}
\newcommand{\flowDirectionExits}{\ensuremath{\flowDirection^{-}}\xspace}
\newcommand{\pressUBExitFG}[1]{\ensuremath{\ub{\press}_{#1}^{\mathrm{exit}}}\xspace}

%%-----------------------------------------------------------
%% Mode variables
%%----------------------------------------------------------
\newcommand{\mode}{\ensuremath{m}\xspace}
\newcommand{\modeOp}[1]{\ensuremath{\mode_{#1}^\mathrm{op}}\xspace}
\newcommand{\modeCl}[1]{\ensuremath{\mode_{#1}^\mathrm{cl}}\xspace}
\newcommand{\modeBy}[1]{\ensuremath{\mode_{#1}^\mathrm{by}}\xspace}
\newcommand{\modeAc}[1]{\ensuremath{\mode_{#1}^\mathrm{ac}}\xspace}
\newcommand{\modeCv}[1]{\ensuremath{\mode_{#1}^\mathrm{cvcl}}\xspace} % closed because of a check valve
\newcommand{\modeFix}[1]{\ensuremath{\mode_{#1}^\mathrm{fix}}\xspace} % fixed mode for non-controllable regulators
\newcommand{\modeX}[1]{\ensuremath{\mode_{#1}^\mathrm{x}}\xspace}
\newcommand{\cfg}[1]{\ensuremath{\mode_{#1}^\mathrm{cf}}\xspace}
\newcommand{\opMode}[1]{\ensuremath{\mode_{#1}^\mathrm{om}}\xspace}
\newcommand{\flowDir}[1]{\ensuremath{\mode_{#1}^\mathrm{fd}}\xspace}


%%-----------------------------------------------------------
%% Mode specific pressure and flow variables
%%----------------------------------------------------------
\newcommand{\pressBy}[1]{\ensuremath{\pressI{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowBy}[1]{\ensuremath{\mFlowI{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgL}[1]{\ensuremath{\pressI{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgR}[1]{\ensuremath{\pressI{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfg}[1]{\ensuremath{\mFlowI{#1}^\mathrm{cf}}\xspace}
%% upper bounds for all of them
\newcommand{\pressByUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRUB}[1]{\ensuremath{\pressUB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgUB}[1]{\ensuremath{\mFlowUB{#1}^\mathrm{cf}}\xspace}
%% lower bounds for all of them
\newcommand{\pressByLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{by}}\xspace}
\newcommand{\mFlowByLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{by}}\xspace}
\newcommand{\pressClLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cl}}\xspace}
\newcommand{\pressClRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cl}}\xspace}
% there is no closed flow, it's zero
\newcommand{\pressCfgLLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{l-cf}}\xspace}
\newcommand{\pressCfgRLB}[1]{\ensuremath{\pressLB{#1}^\mathrm{r-cf}}\xspace}
\newcommand{\mFlowCfgLB}[1]{\ensuremath{\mFlowLB{#1}^\mathrm{cf}}\xspace}

%%-----------------------------------------------------------
%% Slack variables
%%----------------------------------------------------------
\newcommand{\slack}{\ensuremath{\sigma}\xspace}
\newcommand{\slackPPos}[1]{\ensuremath{\slack_{#1}^{\press+}}\xspace}
\newcommand{\slackPNeg}[1]{\ensuremath{\slack_{#1}^{\press-}}\xspace}
\newcommand{\slackQPos}[1]{\ensuremath{\slack_{#1}^{\inflow+}}\xspace}
\newcommand{\slackQNeg}[1]{\ensuremath{\slack_{#1}^{\inflow-}}\xspace}

%%-----------------------------------------------------------
%% Target values
%%----------------------------------------------------------
%% target value types
\newcommand{\PIN}{\pressI{\mathrm{in}}\xspace}
\newcommand{\POUT}{\pressI{\mathrm{out}}\xspace}
\newcommand{\MINPIN}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MAXPIN}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\PIN\,}}\xspace}
\newcommand{\MINPOUT}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MAXPOUT}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\POUT\,}}\xspace}
\newcommand{\MINQ}{\ensuremath{\underbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\MAXQ}{\ensuremath{\overbracket[0.1ex][0.22ex]{\,\mFlow\,}}\xspace}
\newcommand{\SETQ}{\ensuremath{\mFlowI{\mathrm{set}}}\xspace}

%% sets
\newcommand{\setTargetValues}{\ensuremath{\Gamma}\xspace} % all TVs
\newcommand{\setTargetValuesI}[1]{\ensuremath{\setTargetValues_{#1}}\xspace} % ... of some element
\newcommand{\setStaPush}{\ensuremath{\Theta}\xspace} % all stable/pushing TV combinations
\newcommand{\setStaPushI}[1]{\ensuremath{\setStaPush_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushActive}{\ensuremath{\setStaPush^\mathrm{ac}}\xspace} % all combinations for active mode
\newcommand{\setStaPushActiveI}[1]{\ensuremath{\setStaPushActive_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushBypass}{\ensuremath{\setStaPush^\mathrm{by}}\xspace} % all combinations for bypass mode
\newcommand{\setStaPushBypassI}[1]{\ensuremath{\setStaPushBypass_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushClosed}{\ensuremath{\setStaPush^\mathrm{cl}}\xspace} % all combinations for closed mode
\newcommand{\setStaPushClosedI}[1]{\ensuremath{\setStaPushClosed_{#1}}\xspace} % ... of some element
\newcommand{\setStaPushXI}[1]{\ensuremath{\setStaPush^\mathrm{x}_{#1}}\xspace} % all combination for x mode for some element
\newcommand{\setTVBPolysI}[1]{\ensuremath{\Phi_{#1}}\xspace}
\newcommand{\setTVBPolysActiveI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac}}\xspace}
\newcommand{\setTVBPolysBypassI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{by}}\xspace}
\newcommand{\setTVBPolysClosedI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{cl}}\xspace}
\newcommand{\setTVBPolysActiveQI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}Q}}\xspace}
\newcommand{\setTVBPolysActivePInI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{in}}}\xspace}
\newcommand{\setTVBPolysActivePOutI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}p_{out}}}\xspace}
\newcommand{\setTVBPolysActiveXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{ac\text{-}X}}\xspace}
\newcommand{\setTVBPolysXI}[1]{\ensuremath{\setTVBPolysI{#1}^\mathrm{X}}\xspace}
\newcommand{\setTVQuantities}{\ensuremath{\Omega}\xspace}

%% vars
\newcommand{\tv}{\ensuremath{\tau}\xspace}
\newcommand{\tvI}[1]{\ensuremath{\tv_{#1}}\xspace}
\newcommand{\lbTVI}[1]{\ensuremath{\lb{\tv}_{#1}}\xspace}
\newcommand{\ubTVI}[1]{\ensuremath{\ub{\tv}_{#1}}\xspace}

% set values

\newcommand{\tvSet}{\ensuremath{\tv^\mathrm{set}}\xspace}
\newcommand{\tvSetI}[1]{\ensuremath{\tvSet_{#1}}\xspace}

%\newcommand{\varMINPIN}[2]{\ensuremath{\tv^{\MINPIN}_{#1,#2}}\xspace}
%\newcommand{\varMAXPIN}[2]{\ensuremath{\tv^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\varMINPOUT}[2]{\ensuremath{\tv^{\MINPOUT}_{#1,#2}}\xspace}
%\newcommand{\varMAXPOUT}[2]{\ensuremath{\tv^{\MAXPOUT}_{#1,#2}}\xspace}
%\newcommand{\varMINQ}[2]{\ensuremath{\tv^{\MINQ}_{#1,#2}}\xspace}
%\newcommand{\varMAXQ}[2]{\ensuremath{\tv^{\MAXQ}_{#1,#2}}\xspace}
%
%% not complete yet ...
%\newcommand{\lbMAXPIN}[2]{\ensuremath{\lb{\tv}^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\ubMAXPIN}[2]{\ensuremath{\ub{\tv}^{\MAXPIN}_{#1,#2}}\xspace}
%\newcommand{\lbMINPOUT}[2]{\ensuremath{\lb{\tv}^{\MINPOUT}_{#1,#2}}\xspace}
%\newcommand{\ubMINPOUT}[2]{\ensuremath{\ub{\tv}^{\MINPOUT}_{#1,#2}}\xspace}

% target value stable pushing combination variable
\newcommand{\tvCombiI}[1]{\ensuremath{\theta_{#1}}\xspace}
% target value bound polytope variable
\newcommand{\tvPolyI}[1]{\ensuremath{\phi_{#1}}\xspace}

\newcommand{\funcTvPrio}{\ensuremath{\varphi}\xspace} % target value priority function
\newcommand{\funcTvPrioI}[1]{\ensuremath{\funcTvPrio(#1)}\xspace} % .. with argument


%%-----------------------------------------------------------
%% Objective change variables
%%----------------------------------------------------------
\newcommand{\objVar}{\ensuremath{\delta}\xspace}
\newcommand{\objVarI}[1]{\ensuremath{\delta_{#1}}\xspace}
\newcommand{\opModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{om}}}\xspace}
\newcommand{\unitStart}[1]{\ensuremath{\objVarI{#1}^{\mathrm{us}}}\xspace}
\newcommand{\regModeChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg}}}\xspace}
\newcommand{\xPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pl}}}\xspace}
\newcommand{\xPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-pr}}}\xspace}
\newcommand{\xQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{X-q}}}\xspace}
\newcommand{\rgPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pl}}}\xspace}
\newcommand{\rgPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-pr}}}\xspace}
\newcommand{\rgQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{rg-q}}}\xspace}
\newcommand{\csPLChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pl}}}\xspace}
\newcommand{\csPRChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-pr}}}\xspace}
\newcommand{\csQChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{cs-q}}}\xspace}
\newcommand{\tvChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{tv}}}\xspace}
\newcommand{\tvSetChg}[1]{\ensuremath{\objVarI{#1}^{\mathrm{set}}}\xspace}

%%-----------------------------------------------------------
%% Objective cost parameters
%%-----------------------------------------------------------
\newcommand{\cost}{\ensuremath{w}\xspace}
\newcommand{\costSlackP}{\ensuremath{\cost^{\slack\mathrm{-p}}}\xspace}
\newcommand{\costSlackQ}{\ensuremath{\cost^{\slack\mathrm{-d}}}\xspace}
\newcommand{\costOpModes}{\ensuremath{\cost^\mathrm{om}}\xspace}
\newcommand{\costUnitStarts}{\ensuremath{\cost^\mathrm{us}}\xspace}
\newcommand{\costRgModeChg}{\ensuremath{\cost^\mathrm{rg}}\xspace}
\newcommand{\costXPLChg}{\ensuremath{\cost^\mathrm{X-pl}}\xspace}
\newcommand{\costXPRChg}{\ensuremath{\cost^\mathrm{X-pr}}\xspace}
\newcommand{\costXQChg}{\ensuremath{\cost^\mathrm{X-q}}\xspace}
\newcommand{\costRgPLChg}{\ensuremath{\cost^\mathrm{rg-pl}}\xspace}
\newcommand{\costRgPRChg}{\ensuremath{\cost^\mathrm{rg-pr}}\xspace}
\newcommand{\costRgQChg}{\ensuremath{\cost^\mathrm{rg-q}}\xspace}
\newcommand{\costCsPLChg}{\ensuremath{\cost^\mathrm{cs-pl}}\xspace}
\newcommand{\costCsPRChg}{\ensuremath{\cost^\mathrm{cs-pr}}\xspace}
\newcommand{\costCsQChg}{\ensuremath{\cost^\mathrm{cs-q}}\xspace}
\newcommand{\costFlowDirectionChange}{\ensuremath{\cost^f}\xspace}
\newcommand{\costFlowDirectionChangeNaviStation}[1]{\ensuremath{\costFlowDirectionChange_{#1}}\xspace}
\newcommand{\costOriginalSimpleStateChange}{\ensuremath{\tilde{\cost}^s}\xspace}
\newcommand{\costSimpleStateChange}{\ensuremath{\cost^s}\xspace}
\newcommand{\costArtificialLinkChange}{\ensuremath{\cost^a}\xspace}
\newcommand{\costCompressingLinkOn}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-act}}}\xspace}
\newcommand{\costCompressingLinkValue}[1]{\ensuremath{\cost_{#1}^{\mathrm{cp-val}}}\xspace}
\newcommand{\costSmoothingPressure}{\ensuremath{\cost^{\mathrm{sm-p}}}\xspace}
\newcommand{\costSmoothingFlow}{\ensuremath{\cost^{\mathrm{sm-q}}}\xspace}
\newcommand{\costTVChg}{\ensuremath{\cost^\mathrm{tv}}\xspace}

%%-----------------------------------------------------------
%% Other physical quantities
%%----------------------------------------------------------
\newcommand{\velo}{\ensuremath{v}\xspace}
\newcommand{\absVelo}[1]{\ensuremath{|\velo_{#1}|}\xspace}
\newcommand{\gasConst}{\ensuremath{R}\xspace}
\newcommand{\sGasConst}{\ensuremath{\gasConst_{\mathrm{s}}}\xspace}
\newcommand{\temp}{\ensuremath{T}\xspace}
\newcommand{\tempI}[1]{\ensuremath{\temp{#1}}\xspace}
\newcommand{\zFact}{\ensuremath{z}\xspace}
\newcommand{\zFactI}[1]{\ensuremath{\zFact_{#1}}\xspace}
\newcommand{\vol}{\ensuremath{V}\xspace}
\newcommand{\amountOfSubstance}{\ensuremath{n}\xspace}
\newcommand{\pseudoP}{\ensuremath{\press^\mathrm{c}}\xspace}
\newcommand{\pseudoT}{\ensuremath{\temp^\mathrm{c}}\xspace}
\newcommand{\molMass}{\ensuremath{M}\xspace}
\newcommand{\len}{\ensuremath{L}\xspace}
\newcommand{\lenI}[1]{\ensuremath{\len_{#1}}\xspace}
\newcommand{\area}{\ensuremath{A}\xspace}
\newcommand{\areaI}[1]{\ensuremath{\area_{#1}}\xspace}
\newcommand{\diam}{\ensuremath{D}\xspace}
\newcommand{\diamI}[1]{\ensuremath{\diam_{#1}}\xspace}
\newcommand{\slope}{\ensuremath{s}\xspace}
\newcommand{\slopeI}[1]{\ensuremath{\slope_{#1}}\xspace}
\newcommand{\fric}{\ensuremath{\lambda}\xspace}
\newcommand{\fricI}[1]{\ensuremath{\fric_{#1}}\xspace}
\newcommand{\rough}{\ensuremath{k}\xspace}
\newcommand{\roughI}[1]{\ensuremath{\rough_{#1}}\xspace}
\newcommand{\dynVisc}{\ensuremath{\eta}\xspace}
\newcommand{\gravAcc}{\ensuremath{g}\xspace}
\newcommand{\dens}{\ensuremath{\rho}\xspace}
\newcommand{\nDens}{\ensuremath{\dens_0}\xspace} % subscript is used in the code for this and should be left free, if possible
\newcommand{\vFlow}{\ensuremath{Q}\xspace}
\newcommand{\nvFlow}{\ensuremath{Q^0}\xspace}
\newcommand{\nvFlowI}[1]{\ensuremath{Q^0_{#1}}\xspace}
\newcommand{\timeDiff}{\ensuremath{\Delta_t}\xspace} %equals \tau(t) - \tau(t-1)
\newcommand{\power}{\ensuremath{P}\xspace}
\newcommand{\adEnth}{\ensuremath{H_\mathrm{ad}}\xspace}
\newcommand{\adEff}{\ensuremath{\eta_\mathrm{ad}}\xspace} % \eta is already the dyn viscosity, but it's the same in the gas book
\newcommand{\isenExp}{\ensuremath{\kappa}\xspace}

%%-----------------------------------------------------------
%% Other element parameters
%%----------------------------------------------------------
\newcommand{\height}[1]{\ensuremath{h_{#1}}\xspace}
\newcommand{\drag}[1]{\ensuremath{\zeta_{#1}}\xspace}
\newcommand{\machinePDiffUB}{\ensuremath{\ub{\Delta}_\press}\xspace}

%%-----------------------------------------------------------
%% Number sets
%%----------------------------------------------------------
\newcommand{\setReals}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\setRealsNonNeg}{\ensuremath{\setReals_{\geq 0}}\xspace}
\newcommand{\setRealsNonPos}{\ensuremath{\setReals_{\leq 0}}\xspace}
\newcommand{\setRealsNeg}{\ensuremath{\setReals_{< 0}}\xspace}
\newcommand{\setRealsPos}{\ensuremath{\setReals_{> 0}}\xspace}
\newcommand{\setNaturalNumbers}{\ensuremath{\mathbb{N}}\xspace}
